Modelling and Search-Based Testing of Robot Controllers Using Enzymatic Numerical P Systems

The safety of the systems controlled by software is a very important area in a digitalized society, as the number of automated processes is increasing. In this paper, we present the results of testing the accuracy of different lane keeping controllers for an educational robot. In our approach, the robot is controlled using numerical P systems and enzymatic numerical P systems. For tests generation, we used an open-source tool implementing a search-based software testing approach.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{H. Cheval, L. Leu\c{s}tean, A. Sipo\c{s} (Eds.):\\ 7th Symposium on Working Formal Methods (FROM 2023)\\
EPTCS 389, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.389.1}{10.4204/EPTCS.389.1}}
\pdfoutput=1

